Understanding and Mitigating the Tradeoff Between Robustness and Accuracy

Adversarial training augments the training set with perturbations to improve the robust error (over worst-case perturbations), but it often leads to an increase in the standard error (on unperturbed test inputs). Previous explanations for this tradeoff rely on the assumption that no predictor in the hypothesis class has low standard and robust error. In this work, we precisely characterize the effect of augmentation on the standard error in linear regression when the optimal linear predictor has zero standard and robust error. In particular, we show that the standard error could increase even when the augmented perturbations have noiseless observations from the optimal linear predictor. We then prove that the recently proposed robust self-training (RST) estimator improves robust error without sacrificing standard error for noiseless linear regression. Empirically, for neural networks, we find that RST with different adversarial training methods improves both standard and robust error for random and adversarial rotations and adversarial $\ell_\infty$ perturbations in CIFAR-10.

==> app-variance.tex <==
\section{Variance of minimum norm interpolants}
\label{sec:app-variance}

In this section, we consider the case where the noise is non-zero, and compute the variances of the two estimators of interest: the standard estimator $\stdest$ and data augmented estimator $\augest$.
The following theorem provides a general characterization of the relation between variance of the standard estimator and variance of the augmented estimator.
Theorem~\ref{thm:simple-variance} is a corollary of this general result that we present first. 
\begin{restatable}[Variance]{theorem}{firstvariance}
  \label{thm:appendix-variance}
  The difference in the variances of a standard and augmented estimator can be expressed as follows:
  \begin{align}
\label{eqn:general-variance}
   \frac{1}{\sigma^2}(V(\augest) - V(\stdest))&= \underbrace{\tr\big( \sigmapop \pinvxextperp (\pinvxextperp)^\top \big)}_{\text{$T_1$: Variance increase}}
    - \underbrace{\tr\big( \sigmapop \sigmastd^\dagger \xext^\top(I + \xext \sigmastd^\dagger \xext^\top)^{-1} \xext \sigmastd^{\dagger}\big)}_{\text{$T_2$: Variance reduction}},
  \end{align}
  where $\xextperp \eqdef \pistd \xext$, is the component of $\xext$ in the null space of $\sigmastd$.
\end{restatable}

\begin{proof}
  Recall from~\refeqn{bias-variance} that the $V(\hat{\theta}) = \tr(\cov(\hat{\theta} \mid \xstd \xext)\sigmapop)$. For the minimum norm interpolation estimators $\stdest$ and $\augest$ in Equation~\ref{eqn:est}, we have the following expressions for the variances of the estimators. 
  \begin{align*}
    V(\stdest)&= \sigma^2 \tr\Big( \sigmastd^{\dagger} \sigmapop\Big),  \\
    V(\augest)&= \sigma^2 \tr\Big( \sigmaaug^{\dagger} \sigmapop\Big),
  \end{align*}
  where $\sigmastd = \xstd^\top \xstd$ and $\sigmaaug = \xstd^\top \xstd + \xext^\top \xext$.
  Note that since $\sigmastd, \sigmaaug$ are unnormalized, the quantities $\sigmastd^\dagger$
  and $\sigmaaug^\dagger$ decay with $n$ with the variances $V(\stdest), V(\augest)$ also decay with $n$ as expected.  
  In order to compare $V(\stdest)$ and $V(\augest)$, we need to compare $\sigmastd^{\dagger}$
  and $\sigmaaug^{\dagger}$.  Iorder to do this, we leverage the result from~\cite{kovanic1979pseudoinverse} on the pseudo-inverse of the sum of two symmetric matrices:
  \begin{align*}
    (\sigmastd + \xext^\top \xext)^{\dagger} &= \sigmastd^{\dagger} - \sigmastd^\dagger \xext^\top(I + \xext \sigmastd^\dagger \xext^\top)^{-1} \xext \sigmastd^{\dagger} + \pinvxextperp (\pinvxextperp)^\top,
  \end{align*}
  where recall that $\xextperp$ % \eqdef (I - \hatsigmaorig \hatsigmaorig^\dagger) \xaug=\hatpiorig \xaug$
  is the component of $\xext$ in the null space of $\sigmastd$. Multiplying each term by $\sigmapop$ and using linearity of trace, we get the required expression.
\end{proof}

\paragraph{Proof of Theorem~\ref{thm:simple-variance}}. Theorem~\ref{thm:simple-variance} follows directly from the general result above (Theorem~\ref{thm:appendix-variance}). Note that the terms $T_1$ and $T_2$ are traces of PSD matrices and hence non-negative,
and capture the magnitude of variance increase and variance reduction respectively. 
From Theorem~\ref{thm:appendix-variance}, we see that (i) if $\xext$ is entirely in the span of $\sigmastd$ making $\xextperp = 0$, $T_1 = 0$ making $V(\augest) \leq V(\stdest)$ (ii) On the other extreme, if $\xext$ is entirely in the null space with $\sigmastd^\dagger \xext = 0$, $T_2 = 0$ and hence $V(\augest) \geq V(\stdest)$.

